Explaining Preferences with Shapley Values

While preference modelling is becoming one of the pillars of machine learning, the problem of preference explanation remains challenging and underexplored. In this paper, we propose \textsc{Pref-SHAP}, a Shapley value-based model explanation framework for pairwise comparison data. We derive the appropriate value functions for preference models and further extend the framework to model and explain \emph{context specific} information, such as the surface type in a tennis game. To demonstrate the utility of \textsc{Pref-SHAP}, we apply our method to a variety of synthetic and real-world datasets and show that richer and more insightful explanations can be obtained over the baseline.

==> contents/00_direction.tex <==
\section*{How are we going to present the stories?}

Consider the following duelling setup: we have $n$ items, each with $d$ covariates $\bfx \in \RR^{n \times d}$. We assume there are $T$ number of pairwise comparisons made, and we encode these in the following way: 
\begin{align}
    r_t = 
    \begin{cases}
    1 & \text{if } x_t \succ x_t' \\
    -1 & \text{if } x_t' \succ x_t \\
    0 & \text{otherwise}
    \end{cases}
\end{align}
where $r_t$ denotes the preference of item $x_t$ to $x'_t$. There are different ways to model this problem, depending on the available covariate information about the items and the comparisons themselves.

\subsubsection*{A. Ranking} In the simplest case when there are no items' covariates, we could utilise classical probabilistic ranking algorithms such as Bradley-Terry model or spectral algorithms such as rank centrality, serial rank or SVD Rank, to learn a 1-d skill vector, which can then be used to infer rankings. When there are item covariates, we could use preferential GP or SVDRankCov to learn the ranking as a function of the covariates.

\paragraph{What does explainability mean in this case?} We are interested to know what item covariates lead to this particular 1-d skill vector. \textbf{However, when there are no player covariates, can we still get some explanations to why we are seeing what we have seen?} The answer is yes, and it only requires a minimal modification to an existing algorithm. To do this, we set up the following similarity graph,
\begin{align}
    \bfS = \frac{1}{2}(n \bfone \bfone^\top + \bfC\bfC^\top)
\end{align}
and utilise this as features for our modelling. This allows us to answer questions of this type: "What are the most influential matches corresponds to this particular rank for player $x$?"


\subsubsection*{B. Preference Learning} Ranking gives us the simplest way to deduce preferences by referring to the order of each item in the rank. However, when preferences are inconsistent to one underlying total ordering, one might just be better off by modelling the preference directly, i.e. learning the function $g(x, x')$ that tells you the preference of $x$ over $x'$. This is more interesting when we have external covariates governing the comparisons itself, for example a covariate $u$ such that the preference of $x$ over $x'$ at condition $u$ is modelled by $g(u, x, x')$.

\paragraph{What does explainability mean in this case?} For a particular comparison, what are the factors that constitute this outcome?

==> contents/01_intro_by_robert.tex <==
% \section{Introduction}

% \emph{Preference learning}~\cite{10.1007/978-3-540-39857-8_15} is a classical problem in machine learning, where one is interested in learning the order relations on a collection of data items.  This class of algorithms~\citep{bradley1952rank,thurstone1994law,chu2005preference,gonzalez2017preferential} often assume there is a latent scaler utility function $f$ that dictates the outcome of preferences. For example, explicit feedbacks such as item ratings or rankings from recommender systems can be treated as noisy evaluations of $f$, whereas pairwise comparison data from sports~\cite{} or duelling games~\cite{chau2020spectral} can be used to implicitly infer $f$, i.e. player $\bfxleft$ is preferred over (beats) player $\bfxright$ when $f(\bfxleft) > f(\bfxright)$. However, as \citet{chau2020learning} discussed, explicit direct feedback from $f$ is often scarce or expensive, and the quantity of implicit feedback data typically far outweighs the explicit data. Moreover, when the feedback is from human,~\citet{kahneman1979interpretation} showed that they are better at evaluating relative differences than absolute quantities. Motivated by such, in this paper, we will focus on modelling, and particularly, explaining preferences inferred using duelling data.



% \emph{Preference learning} \cite{10.1007/978-3-540-39857-8_15} is a classical problem in machine learning, where one tries to learn the pairwise preference function $f$ between objects $x_i$ and $x_j$, where $x_i$ is preferred over $x_j$ if $f(x_i)>f(x_j)$. These days, it is often seen as the predecessor to \emph{Learning to rank} \cite{10.1145/1273496.1273513}, where one instead directly learns a list or ranked items directly rather than inferring them from pairwise comparisons.
% % \vspace{-0.2cm}
% \begin{wrapfigure}[22]{r}{0.4\textwidth}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{teaserplot/bee_plot_lamb=0.0_lasso.png}
%         \includegraphics[width=0.4\textwidth]{teaserplot/bar_plot_lamb=0.0_lasso.png}
%   \end{center}
%     \vspace{-10pt}
%   \caption{\textsc{Pref-SHAP} finds the importance of speed and type advantage between water and fire Pokémon battles!}
% \end{wrapfigure}
% \emph{Preference learning} and, by extension, \emph{Learning to rank} assumes that all items, given any query is \emph{rankable}, meaning one assumes there exists a true exact ordering of all items. As an example, if a user queries what movies to watch, one would assume that the user can exactly write down the specific order of movies preferred when given a list. From the example alone, many practical questions arise such as: ``Doesn't this require that the user both knows all movies that are offered together with having an intrinsic consistent scoring rule for all movies?''. Despite this strong assumption, preference learning has had many successful instantiations in  \citep{chu2005preference, d2019ranking, gonzalez2017preferential, houlsby2012collaborative}. 

% However nature often violates the assumptions of rankability \cite{sinervo1996,PERVAN2015726,10.1086/208573}, e.g. preference of $A$ over $B$, $B$ over $C$, but $C$ over $A$ -- thus conforming to the \emph{rock-paper-scissors relation}. Such \emph{inconsistent preferences} are under frequent study in social choice theory \citep{sep-social-choice,gehrlein1983condorcet}, but is of wider interest in both healthcare \cite{pref_learning_medicine} and retail \cite{retail_pref} where data is both large and noisy.

% Recently \cite{chau2020learning} proposed \emph{Generalized Preferential Gaussian Process} (GPGP) to learn the aforementioned inconsistent preferences, obtaining state-of-art performance on non-rankable problems. While accurate predictions are generally useful, safety critical applications of machine learning such as healthcare often requires model interpretability.

% While many existing interpretability frameworks \cite{lundberg2017unified,lime} can be directly applied to ranking methods, there currently does not exist methods to explain inconsistent preferences in GPGP. This absence is owed to GPGP being a bi-input kernel method, a treacherous combination of properties overlooked by the interpretability literature. All is not lost however, as \cite{chau2021rkhs} recently proposed RKHS-SHAP to explain single-input kernel methods. With this glimmer of hope, we set out for a perilous journey in explaining inconsistent preferences for GPGP, which we coin \textsc{Pref-SHAP}. We summarize our contributions as follows:

% \begin{enumerate}
%     \item A novel framework coined \textsc{Pref-SHAP} to explain inconsistent preferences on \emph{contest-specific} level, explaining both players and contest environment.
%     \item Empirical demonstrations of \textsc{Pref-SHAP} finding richer insights than just explaining rank on real-world datasets
%     \item A high-performance implementation of \textsc{Pref-SHAP} in [github]
    
% \end{enumerate}

% % Explain why this differs from explaining rank and why explaining inconsistent prefrences is another beast. Start detailing into contributions


% % \begin{wrapfigure}{r}{0.4\textwidth} %replace with others improve explain, other types. 
% %   \begin{center}
% %     \includegraphics[width=0.4\textwidth]{teaserplot/bar_plot_lamb=0.0_lasso.png}
% %   \end{center}
% %     \vspace{-0.1cm}
% %   \caption{}
% % \end{wrapfigure}

% Paper arranged as!


==> contents/03.5_computational_methods.tex <==



% \subsection{Computational considerations for \textsc{Pref-SHAP}}
% We summarize the procedure of \textsc{Pref-SHAP} in Algorithm \ref{main_alg}.
% \begin{algorithm}[htb!]
% \caption{\textsc{Pref-SHAP}}
% \label{main_alg}
% \begin{algorithmic}[1]
% \Require Solution $\boldsymbol{\alpha}$, datasets $\bfXleft,\bfXright,\bfX, \bfU$, test items $\bfxleft,\bfxright,\mathbf{u}$, batch size $n_b$, number of coalition samples $n_S$, context-specific flag $\texttt{cflg}$
% \State Compute effective dimension $d_{\text{eff}}$ := Number of features with variance greater than 0. 
% \State Compute coalitions $\mathcal{S}=\{S_1,\hdots, S_{n_S}\}$, form binary matrix $\mathbf{Z} \in \{0,1\}^{n_S,d_{\text{eff}}}$ from $\mathcal{S}$, and compute weights $\mathbf{W}=[w_1,\hdots,w_{n_S}]$ with $w_i=\frac{d-1}{ {{d}\choose{|S_i|}} |S_i|(d-|S_i|)}$.
% \For { batch $\mathcal{S}_b$ in $\mathcal{S}$}
% \State \textbf{if} \texttt{cflg} Take $S,S^c$ of $\bfXleft,\bfXright,\bfX,\bfxleft,\bfxright$ \textbf{else} Take $S',S'^c$ of $\bfU,\bfu$ 
% \State \textbf{if} \texttt{cflg} Compute $\bfK_{\bfX_S, \lambda}^{-1}[\bfK_{\bfX_S, \bfxleft_S},\bfK_{\bfX_S, \bfxright_S }]$ \textbf{else} $\left(\bfK_{\bfU_{S'}, \bfU_{S'}} + m\lambda' I\right)^{-1}\bfK_{\bfU_{S'}, \bfu_{S'}}$ using \texttt{BatchedCGD}
% \State \textbf{if} \texttt{cflg} Compute $ \hat{\nu}_{\small \bfxleft,\bfxright, \mathcal{S}_b}^{(p)}(\hat{g})$ \textbf{else} $  \hat{\nu}_{\bfu,\bfxleft,\bfxright, \mathcal{S}_b'}(\hat{g}_U)$
% \EndFor
% \State \textbf{if} \texttt{cflg} Set $\mathbf{v}_x=\{ \hat{\nu}_{\small \bfxleft,\bfxright, \mathcal{S}_b}^{(p)}(\hat{g})\}^{B}_{b=1}$ \textbf{else} $\mathbf{v}_x=\{\hat{\nu}_{\bfu,\bfxleft,\bfxright, \mathcal{S}_b'}(\hat{g}_U)\}^{B}_{b=1}$
% \State Calculate Shapley values $\boldsymbol{\beta}_{x}=\left(\mathbf{Z}^{\top}\mathbf{W} \mathbf{Z}\right)^{-1} \mathbf{Z}^{\top} \mathbf{W} \mathbf{v}_{x}$\\
% \Return $\boldsymbol{\beta}_{x}$
% \end{algorithmic}
% \end{algorithm}
% We propose several optimizations in the \textsc{Pref-SHAP} procedure. We consider batched conjugate gradient descent detailed in the Appendix and fast sampling of coalitions $S$ in Algorithm \ref{algo1} described below. \newline 
% \textbf{Fast coalitions} \quad We first propose an optimized sampling scheme for finding coalitions $S$ in Algorithm \ref{algo1}.
% \begin{algorithm}[htb!]
% \caption{Sampling unique $n$, $d$-dimensional coalitions in $\mathcal{O}(d)$ time}
% \label{algo1}
% \begin{algorithmic}[1]
% \Require Number of coalitions $n$, number of features $d$.
% \State $I=\text{SampleWithoutReplacement}(n,0,2^d)$ \Comment{Sample $n$ unique integers between $0$ and $2^d$}
% \Function{\textnormal{base2}}{i}: \Comment{Convert integer to base-2 representation}
% \State $S = [0,\hdots, 0] \in \mathbb{R}^d$, $r=i$ \Comment{Initialize $d$-dimensional 0 vector and the rest term $r$}
% \While {$r>0$}
% \State $i = \lfloor\log_2{(r)}\rfloor$ \Comment{Find which index of $S$ to set to 1}
% \State $S[i]=1$ \Comment{Update $S$}
% \State $r = r -2^{i}$ \Comment{Update rest term}
% \EndWhile
% \State \textbf{return} $S$
% \EndFunction %
% \Return $\{S_1,\hdots S_{n}\}=\text{parallel\_apply}(I,\text{base2})$ \Comment{Each integer can be independently converted}
% \end{algorithmic}
% \end{algorithm}
% In contrast to the implementation in \cite{lundberg2017unified} which samples the weights from $p(Z)$, our method is embarrassingly parallel, which allows for an additional $\mathcal{O}(n)$ reduction. A naive algorithm that compares each sample $S_i$ has complexity $\mathcal{O}(n^2d^2)$ and cannot be parallelized. \newline \textbf{Stabilizing the Shapley value estimation}\quad
% To avoid noise from constant features, we filter out features which have $0$ variance of the data we are explaining, similar to the implementation in SHAP. For the coalition $S$, we simply set filtered out features to $0$. To ensure we get numerically stable Shapley Values, we calculate the inverse using Cholesky decomposition, as we found the regular inverse function provided inconsistent results.  







==> contents/03_method.tex <==
% \vspace{-0.1cm}
% \section{Proposed method: \textsc{Pref-SHAP}}
% \vspace{-0.2cm}
% \label{sec: method}

% In this section, we will present \textsc{Pref-SHAP}, a new Shapley explainability algorithm designed to explain preferences by attributing contribution scores over the item-level covariates and contest-level covariates. We note that one can easily recover 

% \subsection{Preferential value function for items}

% Recall the likelihood model for generalised preference model from Sec.~\ref{sec: preference_learning}:
% \begin{align}
%     p\left(y \mid \bfxleft, \bfxright\right) = \sigma\left(yg\left(\bfxleft, \bfxright\right)\right)
% \end{align}
% with $g:\cX \times \cX\to\RR$ the skew-symmetric function denoting the strength of preference of item $\bfxleft$ over item $\bfxright$. To explain this preference model using Shapley values, we propose the following value function:
% \begin{definition}[Preferential value function for items] Given $g\in\cH$ a preference function, $\left(\bfxleft, \bfxright\right) \in \cX\times \cX$ a pair of items to compare, we define the \textit{preferential value function} as $\nu^{(p)}: \cX \times \cX\times[0,1]^d\times \cH \to \RR$ such that:
% \begin{align}
%     \nu^{(p)}_{\bfxleft, \bfxright, S}(g) = \EE_r\left[g(\{\Xleft_S,\Xleft_{S^c}\},\{\Xright_S,\Xright_{S^c}\})\mid \Xleft_S=\bfxleft_S, \Xright_S=\bfxright_S \right]
% \end{align}
% where expectation is taken over the reference $r\left(\Xleft_{S^c},\Xright_\Sc \mid \Xleft_S=\bfxleft_S, \Xright_S=\bfxright_S\right)$.
% \end{definition}
% Similar to standard value functions, the utility of a feature set $S$ is defined as the impact to the preference model after "removing" contributions from features in $\Sc$, via integration with respect to some reference distribution $r$. Similar to $g$, this value function is skew-symmetric in its first two arguments, i.e. $\pnu(\bfxleft,\bfxright, S, g) = -\pnu(\bfxright,\bfxleft, S, g)$. This is justified, since features that ``encourage'' preference of $\bfxleft$ over $\bfxright$ should naturally be the ones that ``discourage'' preference of $\bfxright$ over $\bfxleft$ to ensure consistency. In this paper, we assume the items are i.i.d sampled from some distribution $p$, and we utilise the observational data distribution as reference as in \cite{frye2020shapley}, i.e. we take $r\left(\Xleft_{S^c},\Xright_\Sc \mid \Xleft_S=\bfxleft_S, \Xright_S=\bfxright_S\right)$ to be $p\left(\Xleft_{S^c}\mid \Xleft_S=\bfxleft_S\right)p\left(\Xright_{S^c}\mid \Xright_S=\bfxright_S\right)$. Although we decide to use the observational distribution as the reference, the forthcoming estimation procedure follow analogously with the marginal distribution approach in \citet{janzing2020feature}.


% \shortparagraph{Empirical estimation of the preferential value function $\nu^{(p)}_{\bfxleft, \bfxright, S}(g)$} While the \textit{preferential value function} is general in the sense that it could be applied to any preference function $g$, we divert our attention to functions in $\cH_{k_E}$, where $k_E$ is the \textit{generalised preferential kernel} introduced in Sec~\ref{sec: preference_learning}. This allows us to adapt the recently introduced \textsc{RKHS-SHAP} to our settings, and we can thus circumvent learning an exponential number of conditional densities as in~\cite{frye2020shapley}. In the following segment, we prove the existence of the Riesz representation of the \textit{preferential value functional}, a necessary step to adapt the \textsc{RKHS-SHAP} framework,
% \begin{proposition}[Preferential value functional for items]
% Let $k$ be a product kernel on $\cX$, i.e. $k(\bfxleft,\bfxright) = \prod_{j=1}^d k^{(j)}(x^{(j)}, x'^{(j)})$. Assume $k^{(j)}$ are bounded for all $j$, then the Riesz representation of the functional $\nu^{(p)}_{\bfxleft, \bfxright, S}$ exists and takes the form:
% \begin{align*}
%     \nu^{(p)}_{\bfxleft, \bfxright, S} = \frac{1}{\sqrt{2}} \left(\cK(\bfxleft, S) \otimes \cK(\bfxright, S) - \cK(\bfxright, S) \otimes \cK(\bfxleft, S)\right)
% \end{align*}
% where $\cK(\bfx, S) = k_{S}(\cdot, \bfx_S)\otimes \mu_{X_{S^c}\mid X_S = \bfx_S}$ and $k_S(\cdot, \bfx_S) = \bigotimes_{j\in S}k^{(j)}(\cdot, x^{(j)})$ is the sub-product kernel defined analogously as $X_S$.

% % \begin{align*}
% % \frac{1}{\sqrt{2}}\Big[(k_{S}(\bfxleft_S)\otimes \mu_{X_{S^c}\mid \bfxleft_S})\otimes (k_S(\bfxright_S)\otimes \mu_{X_{S^c}\mid \bfxright_S}) - (k_S(\bfxright_S)\otimes \mu_{X_{S^c}\mid \bfxright_S}) \otimes (k_S(\bfxleft_S)\otimes \mu_{X_{S^c}\mid \bfxleft_S})\Big]
% % \end{align*}
% \end{proposition}
% All proofs are included in the appendix. Now we can estimate the value function non-parametrically,
% \begin{proposition}[Estimating  $\nu^{(p)}_{\bfxleft,\bfxright, S}$]
% \label{prop: pref-shap_esitmation}
% Given $\hat{g} = \sum_{j=1}^m \alpha_j k_E((\bfxleft_j, \bfxright_j), \cdot)$, datasets $\bfXleft, \bfXright$, test items $\bfxleft, \bfxright$, the preferential value function of test point $\bfxleft, \bfxright$ at coalition $S$ with preference function $\hat{g}$ can be estimated by,
% \begin{align*}
%     \hat{\nu}_{\small \bfxleft,\bfxright, S}^{(p)}(\hat{g}) = \balpha^\top\left(\Gamma(\bfXleft_S, \bfxleft_S)\odot \Gamma(\bfXright_S, \bfxright_S) - \Gamma(\bfXleft_S, \bfxright_S)\odot \Gamma(\bfXright_S, \bfxleft_S)\right)
% \end{align*}
% where $\Gamma(\bfXleft_S, \bfxleft_S) = \bfK_{\bfXleft_S, \bfxleft_S}\odot \bfK_{\bfXleft_{S^c}, \bfX_{S^c}}\bfK_{\bfX_S, \lambda}^{-1}\bfK_{\bfX_S, \bfxleft_S}, \bfK_{\bfX_S, \lambda} = \bfK_{\bfX_S, \bfX_S} + n\lambda I$ and $\balpha = \{\alpha_j\}_{j=1}^m$.
% \end{proposition}

% It is also straightforward to explain items' contribution under the \textit{Context-included Generalised Preference model} introduced in Sec.~\ref{sec: preference_learning}. One could either fix a specific context $\bfu$ and set $g_\bfu(\cdot, \cdot) = g_U(\bfu, \cdot, \cdot)$, or average out over the contexts by setting $g_{avg}(\cdot,\cdot) = \EE_{p(U)}[g_U(U, \cdot, \cdot)]$, and then apply Prop.~\ref{prop: pref-shap_esitmation} to explain item-level contributions. The former approach allows one to explain item-level feature importances relative to a specific context, i.e. which player's attribute is most important in a tennis match when they are playing on a grass court. The latter approach looks at the item-contribution averaged out over all context, i.e. which player's attribute is most important regardless of which court type they are playing on.

% %  \subsection{Contest-specific \textsc{Pref-SHAP}}
% % Besides item-level covariates $\bfx\in \RR^d$, when we have collected contest-level covariates $\bfu \in \cU \subseteq \RR^{d'}$, e.g. field conditions during tennis competitions, it can be incorporated into our preference model. Consider the enriched dataset  $D = \left\{ y_j, \bfu_j, \bfxleft_j, \bfxright_j \right\}_{j=1}^m$, given a kernel $k_U$ defined on context space $\cU$, we model the new preference function $g_U:\cU\times \cX\times \cX \to \RR$ with the following kernel,
% % \begin{align*}
% % \small
% %     k_E^{(U)}\left(\left(\bfu_i, \bfxleft_i, \bfxright_i\right), \left(\bfu_j, \bfxleft_j, \bfxright_j \right)\right) = k_U\left(\bfu_i, \bfu_j\right) k_E\left(\left(\bfxleft_i, \bfxright_i\right), \left(\bfxleft_j, \bfxright_j \right)\right)
% % \end{align*}
% % We note that if $k_U$ is universal and the base kernel of $k_E$ is universal, then the above kernel, which is their product, stays universal~\citep{szabo2017characteristic}. We prove this in the appendix. 
% \vspace{-0.2cm}
% \subsection{Preferential value function for context variables}
% \vspace{-0.2cm}
% Analogously, it is also possible to extend the above paradigm to explain the context variables $U$ by designing the following preferential value function for contexts: 

% \begin{proposition}[Preferential value function for contexts] Given a preference function $g_U\in \cH_{k_E^U}$, denote $\Omega' = \{1,...,d'\}$, then the utility of context features $S'\subseteq \Omega'$ on $\{\bfu, \bfxleft,\bfxright\}$ is measured by $\nu_{\bfu, \bfxleft,\bfxright, S'}(g_U) = \EE[g_U\left(\{\bfu_S, U_{\Sc}\}, \bfxleft,\bfxright\right)\mid U_S=\bfu_S]$ where the expectation is taken over the observational distribution of $U$. Now, given a test triplet ($\bfu, \bfxleft, \bfxright)$, if $\hat{g}_U= \sum_{j=1}^m \alpha_j k_E^U\left((\bfu_j, \bfxleft_j, \bfxright_j), \cdot\right)$, the non-parametric estimator is:
% \begin{align*}
%     \hat{\nu}_{\bfu,\bfxleft,\bfxright, S'}(\hat{g}_U) &= \balpha^\top \left(\left( \bfK_{\bfU_{S'}, \bfu_{S'}} \odot \bfK_{\bfU_{S'^c}, \bfU_{S'^c}}\left(\bfK_{\bfU_{S'}, \bfU_{S'}} + m\lambda' I\right)^{-1}\bfK_{\bfU_{S'}, \bfu_{S'}}\right)\odot \Xi_{\bfxleft,\bfxright} \right)
% \end{align*}
% where $\Xi_{\bfxleft,\bfxright} = \left(\bfK_{\bfXleft, \bfxleft}\odot \bfK_{\bfXright, \bfxright} - \bfK_{\bfXright, \bfxleft}\odot \bfK_{\bfXleft, \bfxright}\right)$.
% \end{proposition}

% % It is also straightforward to compute the item-level covariates' contribution under a specific context $\bfu$ by applying Prop.~\ref{prop: pref-shap_esitmation} to the function $g_{\bfu}(\bfxleft,\bfxright) = g_U(\bfu, \bfxleft, \bfxright)$.
% \subsection{\textsc{Pref-SHAP} Algorithm}
% Now, we are ready 


% % \textcolor{blue}{@Alan: remember to write a short paragraph on how one could "fix" certain environment and ask for explanation.}


% % At times when we have extra covariates to describe the context how items $\bfxleft,\bfxright$ are competing, for example, the field conditions when two tennis players compete, we can naturally incorporate that into the \textit{generalised preferential kernel} $k_E$. Assume we now have some extra context variables $\{\bfu_j\}_{j=1}^m $ for each match, e.g. 












